BAE: BERT-based Adversarial Examples for Text Classification

Modern text classification models are susceptible to adversarial examples, perturbed versions of the original text indiscernible by humans which get misclassified by the model. Recent works in NLP use rule-based synonym replacement strategies to generate adversarial examples. These strategies can lead to out-of-context and unnaturally complex token replacements, which are easily identifiable by humans. We present BAE, a black box attack for generating adversarial examples using contextual perturbations from a BERT masked language model. BAE replaces and inserts tokens in the original text by masking a portion of the text and leveraging the BERT-MLM to generate alternatives for the masked tokens. Through automatic and human evaluations, we show that BAE performs a stronger attack, in addition to generating adversarial examples with improved grammaticality and semantic coherence as compared to prior work.

==> EMNLP 2020 Camera Ready_ BAE/media/algo.tex <==
% \setlength{\dbltextfloatsep}{3pt}
% % \renewcommand{\AlCapSty}[1]{\normalfont\small{\textbf{#1}}\unskip}
% \begin{algorithm}[t!]
% % \small
% \caption{\BAE{-R} \ Pseudocode}
% \label{alg1}
% \SetAlgoLined
% \KwInput{Sentence $\X = [t_1, \dots, t_n]$, ground truth label $y$, classifier model C }
% \KwOutput{Adversarial Example $\X_{adv}$}
% \KwInitial{$\X_{adv} \leftarrow \X$}

% Compute token importance $I_{i} \ \forall \ t_i \in 
% \X$

%  \For{$i$ \ in descending order of $I_i$ }{
%  Insert mask M: \\
%   \qquad $\X_M \leftarrow \X_{adv[1:i-1]}[M]\X_{adv[i+1:n]} $\\
%  Predict top-K tokens $\T$ for M $\in \X_M$ \\
%  $\T \leftarrow$ {\sc FILTER}$(\T)$ \\
%  $\lll = \{\}$ \small{\tcp{python-style dict}}
%   \For{$t \in \T$}{
%     $\lll[t] = \X_{adv[1:i-1]}[t]\X_{adv[i+1:n]}$
%   }

%   \textbf{if} $\exists \ t \in \T \ $ s.t $ \ C(\lll[t]) \neq y$ \textbf{then} \\
%   \quad \textbf{Return:} \ $\X_{adv} \leftarrow \lll[t']$ where
%   $C(\lll[t']) \neq y$,
%   \\ \qquad \qquad \ \ $\lll[t']$ has 
%   maximum similarity with $\X$\\
%   \textbf{else} \\
%   \quad $\X_{adv} \leftarrow \lll[t']$ where $\lll[t']$ causes maximum \\ \quad reduction in probability of $y$ in $C(\lll[t'])$ \\ 
%   \textbf{end if}
%  }
%  \textbf{Return:} $\X_{adv} \leftarrow None$ 
% \end{algorithm}

\setlength{\dbltextfloatsep}{3pt}
\renewcommand{\AlCapSty}[1]{\normalfont\small{\textbf{#1}}\unskip}
\begin{algorithm}[t!]
\small
\caption{\small{ \BAE{-R} \ Pseudocode}}
\label{alg1}
\SetAlgoLined
\KwInput{Sentence $\X = [t_1, \dots, t_n]$, ground truth label $y$, classifier model C }
\KwOutput{Adversarial Example $\X_{adv}$}
\KwInitial{$\X_{adv} \leftarrow \X$}

Compute token importance $I_{i} \ \forall \ t_i \in 
\X$

 \For{$i$ \ in descending order of $I_i$ }{
 $\X_M \leftarrow \X_{adv[1:i-1]}[M]\X_{adv[i+1:n]} $\\
 Predict top-K tokens $\T$ for mask M $\in \X_M$ \\
 $\T \leftarrow$ {\sc FILTER}$(\T)$ \\
 $\lll = \{\}$ \tcp{python-style dict}
  \For{$t \in \T$}{
    $\lll[t] = \X_{adv[1:i-1]}[t]\X_{adv[i+1:n]}$
  }

  \textbf{if} $\exists \ t \in \T \ $ s.t $ \ C(\lll[t]) \neq y$ \textbf{then} \\
  \quad \textbf{Return:} \ $\X_{adv} \leftarrow \lll[t']$ where
   $C(\lll[t']) \neq y$,
   \\ \qquad \qquad \ \ $\lll[t']$ has 
   maximum similarity with $\X$\\
  \textbf{else} \\
  \quad $\X_{adv} \leftarrow \lll[t']$ where $\lll[t']$ causes maximum \\ \quad reduction in probability of $y$ in $C(\lll[t'])$ \\ 
  \textbf{end if}
 }
 \textbf{Return:} $\X_{adv} \leftarrow None$ 
\end{algorithm}

==> EMNLP 2020 Camera Ready_ BAE/tables/ablation.tex <==
\begin{table}[b!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{3}{c}{\textbf{Word-LSTM}} & \multicolumn{3}{c}{\textbf{Word-CNN}} & \multicolumn{3}{c}{\textbf{BERT}} \\ 
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
                                  & \textbf{\A}         & \textbf{\B}        &
               \textbf{\C}        & 
               \textbf{\A}        & \textbf{\B}        &
               \textbf{\C}        &
               \textbf{\A}      & \textbf{\B}
               &
               \textbf{\C}        \\ 
               \midrule
\textbf{MR}                       & 15.1               &  10.1       &   3.1     & 
12.4 & 9.6       & 2.8       &       24.3          &  12.9  & 5.7               \\
\textbf{Subj}                     & 14.4                & 12.3        &    5.1    & 16.2               & 13.8         &  7.4     &    13.9             &   11.4   &     7.5        \\ 
\textbf{TREC}                     & 16.6                & 1.6        &    0.2    & 20.0               & 5.0         &  1.4     &    14.0             &   8.6   &     2.4        \\ \bottomrule
\end{tabular}
}
\vspace{-0.75em}
\caption{
Analyzing relative importance of `Replace' and `Insert' perturbations for \BAE. 
\A \ denotes \% of test instances which are successfully attacked by \BAE{-R/I}, but not \BAE{-R}, i.e. \A \ : $(\BAEfont{R/I})\cap\overline{\BAEfont{R}}$. 
Similarly, \
 \B \ : $(\BAEfont{R/I})\cap\overline{\BAEfont{I}}$  \ and \
\C \ : $(\BAEfont{R/I})\cap\overline{\BAEfont{R}}\cap\overline{\BAEfont{I}}$. 
}
\label{tab:ablation}
\end{table}

==> EMNLP 2020 Camera Ready_ BAE/tables/results_table1.tex <==
\begin{table*}[t]

\begin{center}
% \scriptsize
\resizebox{0.72\linewidth}{!}{
\begin{tabular}{clllll}
\toprule
\multirow{2}{*}{\textbf{Model}}    & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Adversarial}}} & \multicolumn{4}{c}{\textbf{Datasets}}                                                                                                         \\ \cmidrule(l){3-6} 
                                   & \multicolumn{1}{c}{\textbf{Attack}}                                             & \multicolumn{1}{c}{\textbf{Amazon}} & \multicolumn{1}{c}{\textbf{Yelp}} & \multicolumn{1}{c}{\textbf{IMDB}} & \multicolumn{1}{c}{\textbf{MR}} \\ \midrule
\multirow{6}{*}{\textbf{wordLSTM}} & Original                                                         & 88.0                                & 85.0                              & 82.0                              & 81.16                           \\
                                   & \small{TextFooler}                                                       & 31.0 \small{(0.747)}                         & 28.0 \small{(0.829)}                       & 20.0 \small{(0.828)}                       & 25.49 \small{(0.906)}                    \\
                                   & \BAE{-R}                                                            & 21.0 \small{(0.827)}                         & 20.0 \small{(0.885)}                       & 22.0 \small{(0.852)}                       & 24.17 \small{(0.914)}                    \\
                                   & \BAE{-I}                                                            & 17.0 \small{(0.924)}                         & 22.0 \small{(0.928)}                       & 23.0 \small{(0.933)}                       & 19.11 \small{(0.966)}                    \\
                                   & \BAE{-R/I}                                                          & 16.0 \small{(0.902)}                         & 19.0 \small{(0.924)}                       & 8.0 \small{(0.896)}                        & 15.08 \small{(0.949)}                    \\
                                   & \BAE{-R+I}                                                          & \textbf{4.0 \small{(0.848)}}                 & \textbf{9.0 \small{(0.902)}}               & \textbf{5.0 \small{(0.871)}}               & \textbf{7.50 \small{(0.935)}}            \\ \midrule
\multirow{6}{*}{\textbf{wordCNN}}  & Original                                                         & 82.0                                & 85.0                              & 81.0                              & 76.66                           \\
                                   & \small{TextFooler}                                                       & 42.0 \small{(0.776)}                         & 36.0 \small{(0.827)}                       & 31.0 \small{(0.854)}                       & 21.18 \small{(0.910)}                    \\
                                   & \BAE{-R}                                                            & 16.0 \small{(0.821)}                         & 23.0 \small{(0.846)}                       & 23.0 \small{(0.856)}                       & 20.81 \small{(0.920)}                    \\
                                   & \BAE{-I}                                                            & 18.0 \small{(0.934)}                         & 26.0 \small{(0.941)}                       & 29.0 \small{(0.924)}                       & 19.49 \small{(0.971)}                    \\
                                   & \BAE{-R/I}                                                          & 13.0 \small{(0.904)}                         & 17.0 \small{(0.916)}                       & 20.0 \small{(0.892)}                       & 15.56 \small{(0.956)}                    \\
                                   & \BAE{-R+I}                                                          & \textbf{2.0 \small{(0.859)}}                 & \textbf{9.0 \small{(0.891)}}               & \textbf{14.0 \small{(0.861)}}              & \textbf{7.87 \small{(0.938)}}            \\ \midrule
\multirow{6}{*}{\textbf{BERT}}     & Original                                                         & 96.0                                & 95.0                              & 85.0                              & 85.28                           \\
                                   & \small{TextFooler}                                                       & 30.0 \small{(0.787)}                         & 27.0 \small{(0.833)}                       & 32.0 \small{(0.877)}                       & 30.74 \small{(0.902)}                    \\
                                   & \BAE{-R}                                                            & 36.0 \small{(0.772)}                         & 31.0 \small{(0.856)}                       & 46.0 \small{(0.835)}                       & 44.05 \small{(0.871)}                    \\
                                   & \BAE{-I}                                                            & 20.0 \small{(0.922)}                         & 25.0 \small{(0.936)}                       & 31.0 \small{(0.929)}                       & 32.05 \small{(0.958)}                    \\
                                   & \BAE{-R/I}                                                          & \textbf{11.0 \small{(0.899)}}                         & 16.0 \small{(0.916)}                       & 22.0 \small{(0.909)}                       & 20.34 \small{(0.941)}                    \\
                                   & \BAE{-R+I}                                                          & 14.0 \small{(0.830)}               & \textbf{12.0 \small{(0.871)}}              & \textbf{16.0 \small{(0.856)}}              & \textbf{19.21 \small{(0.917)}}           \\ \bottomrule
\end{tabular}
}
\end{center}
\vspace{-1em}
\caption{
Automatic evaluation of adversarial attacks on 4 Sentiment Classification tasks. We report the test set accuracy. The average semantic similarity, between the original and adversarial examples, obtained from USE are reported in parentheses. Best performance, in terms of maximum drop in test accuracy, is highlighted in \textbf{boldface}.}
\label{tab:results1}
\end{table*}

==> EMNLP 2020 Camera Ready_ BAE/tables/results_table2.tex <==
\newfloatcommand{capbtabbox}{table}[][1.23\linewidth]

\begin{figure*}
\begin{floatrow}
\capbtabbox{%
\resizebox{\linewidth}{!}{    
  \begin{tabular}{cllll}
    \toprule
    \multirow{2}{*}{\textbf{Model}}    & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Adversarial}}} & \multicolumn{3}{c}{\textbf{Datasets}}                                                                     \\ \cmidrule(l){3-5} 
                                      & \multicolumn{1}{c}{\textbf{Attack}}                                             & \multicolumn{1}{c}{\textbf{MPQA}} & \multicolumn{1}{c}{\textbf{Subj}} & \multicolumn{1}{c}{\textbf{TREC}} \\ \midrule
    \multirow{6}{*}{\textbf{wordLSTM}} & Original                                                         & 89.43                             & 91.9                              & 90.2                              \\
                                      & \small{TextFooler}                                                       & 48.49 \small{(0.745)}                      & 58.5 \small{(0.882)}                       & 42.4 \small{(0.834)}                       \\
                                      & \BAE{-R}                                                            & 45.66 \small{(0.748)}                      & 50.2 \small{(0.899)}                       & 32.4 \small{(0.870)}                       \\
                                      & \BAE{-I}                                                            & 40.94 \small{(0.871)}                      & 49.8 \small{(0.958)}                       & 18.0 \small{(0.964)}                       \\
                                      & \BAE{-R/I}                                                          & 31.60 \small{(0.820)}                      & 43.1 \small{(0.946)}                       & 20.4 \small{(0.954)}                       \\
                                      & \BAE{-R+I}                                                          & \textbf{25.57 \small{(0.766)}}             & \textbf{29.0 \small{(0.929)}}              & \textbf{11.8 \small{(0.874)}}              \\ \midrule
    \multirow{6}{*}{\textbf{wordCNN}}  & Original                                                         & 89.06                             & 91.3                              & 93.2                              \\
                                      & \small{TextFooler}                                                       & 48.77 \small{(0.733)}                      & 58.9 \small{(0.889)}                       & 47.6 \small{(0.812)}                       \\
                                      & \BAE{-R}                                                            & 44.43 \small{(0.735)}                      & 51.0 \small{(0.899)}                       & 29.6 \small{(0.843)}                       \\
                                      & \BAE{-I}                                                            & 44.43 \small{(0.876)}                      & 49.8 \small{(0.958)}                       & 15.4 \small{(0.953)}                       \\
                                      & \BAE{-R/I}                                                          & 32.17 \small{(0.818)}                      & 41.5 \small{(0.940)}                       & 13.0 \small{(0.936)}                       \\
                                      & \BAE{-R+I}                                                          & \textbf{27.83 \small{(0.764)}}             & \textbf{31.1 \small{(0.922)}}              & \textbf{8.4 \small{(0.858)}}               \\ \midrule
    \multirow{6}{*}{\textbf{BERT}}     & Original                                                         & 90.66                             & 97.0                              & 97.6                              \\
                                      & \small{TextFooler}                                                       & 36.23 \small{(0.761)}                      & 69.5 \small{(0.858)}                       & 42.8 \small{(0.866)}                       \\
                                      & \BAE{-R}                                                            & 43.87 \small{(0.764)}                      & 77.2 \small{(0.828)}                       & 37.2 \small{(0.824)}                       \\
                                      & \BAE{-I}                                                            & 33.49 \small{(0.862)}                      & 74.6 \small{(0.918)}                       & 32.2 \small{(0.931)}                       \\
                                      & \BAE{-R/I}                                                          & 24.53 \small{(0.826)}                      & 64.0 \small{(0.903)}                       & 23.6 \small{(0.908)}                       \\
                                      & \BAE{-R+I}                                                          & \textbf{24.34 \small{(0.766)}}             & \textbf{58.5 \small{(0.875)}}              & \textbf{20.2 \small{(0.825)}}              \\ \bottomrule
    \end{tabular}
    }
}{%
  \caption{Automatic evaluation of adversarial attacks on MPQA, Subj and TREC datasets. Other details follow those from Table~\ref{tab:results1}. All 4 modes of \BAE{} attacks almost always outperform TextFooler.} \label{tab:results2}
}
\centering
    \ffigbox[0.78\linewidth]
    {
    \begin{subfigure}[t]{0.33\textwidth}
        \raisebox{-2cm}{\includegraphics[width=\textwidth]{supplementary/supp_graphs/wordLSTM_trec_0_8.png}}
        \caption{Word-LSTM}
    \end{subfigure}
    \begin{subfigure}[t]{0.33\textwidth}
        \raisebox{-2cm}{\includegraphics[width=\textwidth]{supplementary/supp_graphs/bert_trec_0_8.png}}
        \caption{BERT}
    \end{subfigure}
    
    }
    {
  \caption{Graphs comparing attack effectiveness on the TREC dataset, as a function of maximum \% perturbation to the input.}%
  \label{fig:graphs}
}
\end{floatrow}
\end{figure*}

